A Hierarchical Architecture for Neural Materials

Neural reflectance models are capable of reproducing the spatially-varying appearance of many real-world materials at different scales. Unfortunately, existing techniques such as NeuMIP have difficulties handling materials with strong shadowing effects or detailed specular highlights. In this paper, we introduce a neural appearance model that offers a new level of accuracy. Central to our model is an inception-based core network structure that captures material appearances at multiple scales using parallel-operating kernels and ensures multi-stage features through specialized convolution layers. Furthermore, we encode the inputs into frequency space, introduce a gradient-based loss, and employ it adaptive to the progress of the learning phase. We demonstrate the effectiveness of our method using a variety of synthetic and real examples.

==> fig_inception.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    \hspace{-10pt}
    \begin{tabular}{ccc}
    Ours & Ours + Inception & Reference \\
    \includegraphics[width=0.16\textwidth, trim={1cm 1cm 1cm 1cm},clip]{images/inception/ours_wo_inception_green.png}&
    \includegraphics[width=0.16\textwidth, trim={1cm 1cm 1cm 1cm},clip]{images/inception/ours_w_inception_green.png}&
    \includegraphics[width=0.16\textwidth, trim={1cm 1cm 1cm 1cm},clip]{images/inception/reference_green.png}
    % 
    \end{tabular}
    \caption{Our optional decoder using Inception modules brings up the fine details, such as fiber curves in this cloth example. This makes the network larger, and unfair to evaluate with the baseline, hence we exclude this from "Ours" in the comparison results.}
    \label{fig_ablation_inception}
\end{figure}
